Distantly-Supervised Joint Extraction with Noise-Robust Learning

Joint entity and relation extraction is a process that identifies entity pairs and their relations using a single model. We focus on the problem of joint extraction in distantly-labeled data, whose labels are generated by aligning entity mentions with the corresponding entity and relation tags using a knowledge base (KB). One key challenge is the presence of noisy labels arising from both incorrect entity and relation annotations, which significantly impairs the quality of supervised learning. Existing approaches, either considering only one source of noise or making decisions using external knowledge, cannot well-utilize significant information in the training data. We propose DENRL, a generalizable framework that 1) incorporates a lightweight transformer backbone into a sequence labeling scheme for joint tagging, and 2) employs a noise-robust framework that regularizes the tagging model with significant relation patterns and entity-relation dependencies, then iteratively self-adapts to instances with less noise from both sources. Surprisingly, experiments on two benchmark datasets show that DENRL, using merely its own parametric distribution and simple data-driven heuristics, outperforms large language model-based baselines by a large margin with better interpretability.

==> response.tex <==
% \documentclass[11pt]{article}

% \usepackage[margin=1in]{geometry} % You can adjust the 1in to suit your needs.

% \begin{document}
\onecolumn
% \documentclass[12pt, onecolumn]{article}

% \begin{document}

\textbf{Clarification and Motivation}
Thanks to the reviewers, we've clarified our motivation in both the Introduction---solving the presence of noisy labels arising from both incorrect entity and relation annotations---and each methodology section.
We also add additional explanations for each terminology in both Section 2 and Section 3 to make it more clear for understanding.
Our implementation details including model parameters, prompt design for LLM-ICL, and training setup are illustrated in Appendix~\ref{sec:implementation}.

\textbf{Fair Comparison}
We thank all reviewers for this insightful suggestion. 
In our new submission, we've changed the backbone to BERT to enable a fair comparison with most baselines using BERT PLM.
Our main results (DENRL w/ BERT) still achieve significant improvements in terms of F1 scores over existing DS methods, demonstrating the generalizability of our noise reduction method.
Additionally, we've also extended our evaluation to the T5-base model, and defer the results in Appendix~\ref{sec:backbone_generalizability}.


\textbf{Complexity Analysis}
We thank all reviewers for this insightful suggestion.
We've added a thorough efficiency evaluation in Section~\ref{sec:efficiency}, along with a theoretical complexity analysis of our method, to enable a practicable application of our work.


\textbf{Clarity}
Thanks to the suggestions from reviewers.
In the main methodology part (Section~\ref{sec:denoise}), we now clarify the definition of all confusing terminologies such as relation patterns and target attention configuration.

\textbf{Citation of Related Work}
Thanks to the suggestions from all reviewers.
We acknowledge the contribution of existing literature and cite them in our methodology description:

[1] Wang, W. and Pan, S.J., AAAI 2020. Integrating deep learning with logic fusion for information extraction.

[2] Kirsch, B., Niyazova, Z., Mock, M. and Rüping, S., Workshop of ECML PKDD 2019. Noise Reduction in Distant Supervision for Relation Extraction Using Probabilistic Soft Logic.

[3] Jia, Wei, Dai Dai, Xinyan Xiao, and Hua Wu. ACL 2019. ARNOR: Attention regularization based noise reduction for distant supervision relation classification.


% \end{document}
% \end{multicols}
